Confucius Code Agent: Scalable Agent Scaffolding for Real-World Codebases

Real-world software engineering tasks require coding agents that can operate on massive repositories, sustain long-horizon sessions, and reliably coordinate complex toolchains at test time. Existing research-grade coding agents offer transparency but struggle when scaled to heavier, production-level workloads, while production-grade systems achieve strong practical performance but provide limited extensibility, interpretability, and controllability. We introduce the Confucius Code Agent (CCA), a software engineering agent that can operate at large-scale codebases. CCA is built on top of the Confucius SDK, an agent development platform structured around three complementary perspectives: Agent Experience (AX), User Experience (UX), and Developer Experience (DX). The SDK supports a unified orchestrator with advanced context management for long-context reasoning, a persistent note-taking system for cross-session continual learning, and a modular extension system for reliable tool use. In addition, we introduce a meta-agent that automates the construction, evaluation, and refinement of agents through a build-test-improve cycle, enabling rapid agent development on new tasks and tool stacks. Instantiated on the Confucius SDK using the meta-agent, CCA demonstrates strong performance on real-world software engineering tasks. On SWE-Bench-Pro, CCA achieves a Resolve@1 of 59%, exceeding prior research baselines as well as commercial results, under identical repositories, model backends, and tool access.

==> sections/impact.tex <==
\section*{Impact Statement}

This paper advances the field of machine learning by improving the reliability, extensibility, and controllability of LLM-based coding agents through better \emph{agent scaffolding} (orchestration, memory, and tool-use abstractions). 
While these improvements can increase developer productivity and reduce repetitive engineering work, they may also amplify risks common to software automation: generating insecure code, enabling misuse (e.g., accelerating vulnerability discovery or malware development), and causing unintended side effects when interacting with external systems. We mitigate these risks by emphasizing constrained tool interfaces, structured parsing, bounded execution, and auditable traces that support oversight and debugging, but we acknowledge that responsible deployment still requires access control, sandboxing, and human review for high-stakes changes. 


